A note on a sheaf of real regular functions

Coste and Roy in 1979 defined a structural sheaf on the real Zariski spectrum of a semi-real ring $A$ and asked whether the ring of the global sections is $\sum^{-1}_1 A$ where $\sum_1$ is the multiplicative subset $\{1+\sum_{i=1}^n a_i^2|a_i\in A, n\in N\}$ of $A$. We give a positive answer to this question for real rings and integral domains.

==> reference.tex <==
@book {BCR,
    AUTHOR = {Bochnak, Jacek and Coste, Michel and Roy, Marie-Fran\c{c}oise},
     TITLE = {Real Algebraic Geometry},
    SERIES = {Ergebnisse der Mathematik und ihrer Grenzgebiete (3)},
    VOLUME = {36},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {1998},
     PAGES = {x+430},
}

@incollection {coste-roy,
    AUTHOR = {Coste, Michel and Roy, Marie-Fran\c{c}oise},
     TITLE = {Topologies for real algebraic geometry},
 BOOKTITLE = {Topos theoretic methods in geometry},
    SERIES = {Variuos Publ. Ser.},
    VOLUME = {30},
 PUBLISHER = {Aarhus Univ., Aarhus},
      YEAR = {1979},
     PAGES = {37--100},
}  

@book {hartshorne,
    AUTHOR = {Hartshorne, Robin},
     TITLE = {Algebraic Geometry},
    SERIES = {Graduate Tects in Mathematics, No. 52},
    PUBLISHER = {Springer-Verlag, New York- Heidelberg},
      YEAR = {1977},
     PAGES = {x+496},
}
